When Memory Mappings Attack: On the (Mis)use of the ARM Cortex-M FPB Unit

In recent years we have seen an explosion in the usage of low-cost, low-power microcontrollers (MCUs) in embedded devices around us due to the popularity of Internet of Things (IoT) devices. Although this is good from an economics perspective, it has also been detrimental for security as microcontroller-based systems are now a viable attack target. In response, researchers have developed various protection mechanisms dedicated to improve security in these resource-constrained embedded systems. We demonstrate in this paper these defenses fall short when we leverage benign memory mapped design-for-debug (DfD) structures added by MCU vendors in their products. In particular, we utilize the Flash Patch and Breakpoint (FPB) unit present in the ARM Cortex-M family to build new attack primitives which can be used to bypass common defenses for embedded devices. Our work serves as a warning and a call in balancing security and debug structures in modern microcontrollers.

==> attack/attack.tex <==
We now demonstrate how to utilize the FPB Unit to defeat the anticounterfeiting
mechanism employed in the SEGGER J-Link v10. This device is a popular but
expensive debug probe. Some models cost close to 1000 USD at the time
of writing \cite{segger:jlink_price}. The J-Link v10 is based around an NXP
LPC4322 microcontroller which communicates with the device being debugged
through a standard JTAG interface, and to a computer running
through USB.

A counterfeit device must be able to replicate the data sent through the
JTAG scan chain in order to be able to access the debug functionality of the
target device, as well as the protocol used by the debugger probe to
communicate with the debug software running on the PC. This requires some
reverse engineering effort and thus poses as an initial expense for those who
wish to produce counterfeit or cloned devices. Because the JTAG scan chain is
implemented in silicon as part of the debug infrastructure of the target
device, data sent by the probe to the device being debugged can not change.
However, the protocol to communicate between the J-Link and the computer can
change on software updates adding support for new devices, features, improved
communications, and bug fixes. Developer tools can refuse to work with older
versions of the firmware on the device requiring an updated firmware to be
installed in the debug probe before it can be utilized. This state of flux
requires clone and counterfeit vendors to constantly update their version of
the hardware incurring an ongoing expense.

Alternatively, to produce a clone or counterfeit version of this particular
device is to reverse engineer the target hardware, produce a copy of it,
and copy of the software running on the original device. This way, the major
expense is on the initial reverse engineering effort.
As a result, SEGGER uses a copy protection mechanism that ties to the
\emph{Unique ID} feature of the NXP LPC4322 microcontroller \cite{lpc4322} to
license the software of the J-Link debug probe.

\import{./}{segger.tex}

% \subsection{Generalizing the Attack}
% \import{./}{fpb_dwt.tex}



==> attack/fpb_dwt.tex <==
As previously mentioned, the FPB is sufficient to bypass the firmware copy
protection mechanism used in the SEGGER J-Link debug probe with the objective
of creating clone devices. Our attack is directly tied to the way the J-Link
firmware uses the built-in APIs of the LCP4322 to perform its license check.
Since our success is directly tied to an implementation detail, we now
demonstrate how this attack can be performed in the general case by employing
the DWT.

% As previously explained, the FPB is sufficient to bypass the copy protection
% mechanism used in the SEGGER J-Link. In this particular case, we perform this
% action using a control-flow hijack. However, this is exploits a design feature
% in the LPC4322. We generalize this attack without the need to alter
% control-flow by employing the DWT.

For this, we assume that the Unique ID is loaded from a fixed location in the
memory map of the device. The location and its contents is immutable. We also
assume an Unique ID that is arbitrarily long, that is it can be any number of
bytes in size. We also assume that the Unique ID is stored outside the lower
\SI{0.5}{\gibi\byte} of the address space, otherwise, the FPB can be trivially
used to spoof it through the use of data comparators.

% For this, we assume that the Unique ID is loaded from a fixed memory location
% that is immutable. We assume an arbitrary length Unique ID as well.
% Instructions that load into a register can be monitored and modified by the FPB
% if these reside in program memory. However, the Unique ID values are actually
% stored outside a region of memory that the FPB can monitor.


% \begin{lstlisting}[language=C, style=c]
% 	ldr r0, UID_REG
% 	ldr r1, UID_REG + 4
% 	ldr r2, UID_REG + 8
% 	ldr r3, UID_REG + C
% \end{lstlisting}

% The first two instructions can be monitored and patched by FPB unit since there are two literal data 
% comparators. Hence, the last two instructions are executed without patched. Thus, the way we bypass the
% anti-clone mechanism of J-Link is not working anymore. In this case study, we leverage the FPB unit
% along with DWT unit to archive our goal. We make some assumptions in this experiment:
% \begin{itemize} 
% 	\item The size of Unique ID is 16 bytes. 
% 	\item The microcontroller does not provide the IAP function. 
% 	\item The microcontroller has FPB and DWT unit. 
% \end{itemize}

Recall that the DWT can trap on memory accesses, triggering an interrupt to
DebugMonitor, if necessary. We set up the DWT unit to provide hardware
watchpoints for the addresses where the Unique ID is stored. Once configured,
when the firmware attempts to access this area of memory to obtain the device
ID the DWT will raise an exception which causes the CPU to start executing the
\texttt{DebugMonitor} exception when the CPU is not in halting debug mode.
% since the CPU is running in normal mode and not debug mode
%\footnote{A
%Cortex-M CPU operates in normal mode and switches to debug mode when a JTAG
%probe is connected to the scan chain. Debug events are captured by the debug
%probe when the CPU is in debug mode, otherwise, these are handled by the CPU
%itself.},
% an exception is triggered which causes the CPU to enter handler mode
% and to start executing the DebugMonitor routine.
We can utilize this mechanism in conjunction with the FPB to modify the device
ID as it is being accessed.

% Data Watchpoint and Trace unit is part of debug units of Cortex-M series
% processors. The DWT unit is widely used to provide watchpoints, data tracing
% and system profiling on microcontrollers to assist the debug procedure. Among
% serial debug function DWT unit provides, we choose the hardware watchpoint to
% monitor the specific memory read/write access in this experiment. To setup
% the hardware watchpoint function of DWT unit, there are four major registers
% we need to configure, control register, comparator register, mask register
% and function register. After the configuration, once the monitored memory
% region is read/wrote, the DWT interruption is triggered. In the interruption
% function, we are able to track the stack and analyze the context to leak or
% modify sensitive information. In this scenario, we can leverage the DWT
% interruption to modify the Unique ID. 


% Combining the information together, we propose a attack chain to bypass
% potential anti-copy mechanism by faking stored Unique ID. With the FPB/DWT
% attack, we are able to do the data flow hijack in a more general way. We design
% a fake DWT interruption function to replace the original one. Furthermore, we
% configure the DWT unit to hardware watchpoint mode to monitor the read/write
% access of Unique ID region. Then we setup the FPB function to hijack the
% original DWT interruption function to our fake DWT interruption. Thus, each
% time the Unique ID has been read, our fake DWT interruption is triggered. In
% the interruption, we are able to modify the stack and change the Unique ID. We
% explain the details of this attack in the following paragraph and sample codes. 

We first write a new function which examines accesses to the area where the
Unique ID is stored. This function also dynamically remaps unused DWT
comparator registers to cover different areas on the Unique ID storage area as
required. For example, if using a DWT implementation that only offers four
comparator registers and we are overriding an eight word Unique ID, when the
software traps on access to the second word of the Unique ID we set up the
first DWT comparator to point to the fifth word.

We then set the FPB to patch the instruction at the entry of the DebugMonitor
interrupt service handler with a branch to our previously crafted function. We
list the simplified procedures in Appendix \ref{sec:gen_attack}.
We assemble this code and combine it with the firmware which uses the
Unique ID feature. We allow our \texttt{initialize\_system()} function to
execute first by modifying the entry point of the application, recomputing any
static checksums if necessary. Upon power-on, our function executes, setting up
the DWT and FPB with the initial configuration. As the firmware attempts to
access the Unique ID, the DWT intercepts these accesses through our injected
DebugMonitor exception and modifies the obtained values returning the spoofed
Unique ID.

% We assemble this code and place it into an unused region of flash memory.  We
% inject the code using a debug probe into the microcontroller, once again
% modifying the reset vector to point to our initialization code. When the
% microcontroller powers on, the reset handler executes. This sets up the FPB and
% DWT in the required initial configuration. Since the firmware is not modified,
% verification passes, and as it tries to access the Unique ID, the DWT
% intercepts these accesses and our code modifies the obtained values.

% With this, we no longer rely on the implementation characteristics that NXP and
% SEGGER utilize in their products. Instead, we are able to override any loads
% done from the area where the Unique ID is stored using the DWT comparators.

% \ding{172}Design a new DWT interruption function which we implement the Unique
% ID modification feature inside.  We compile this function and program it into
% blank flash region.\newline

% \indent\ding{173}Design a new function. In this function, we configure the DWT
% unit into hardware watchpoint mode and monitor the Unique ID region. Thus the
% comparator register is the address of Unique ID  the Furthermore, we configure
% the FPB unit to patch the address of original DWT interruption function into
% our fake DWT interruption function address. We compile the function and also
% program it into blank flash region.\newline


%\indent\ding{174}By using the programmer, we patch the reset handler of the
%boot loader on microcontroller which is only 4 bytes. The patched reset handler
%is the address of our fake FPB/DWT configuration function. Thus, each time the
%microcontroller is power on, the FPB/DWT unit work together and monitor the
%sensitive information, which is Unique ID in this case. 

% We demonstrate our work with following simplified C code and simulate this
% attack based on STM32F407 chip. We store a Unique ID in flash and use memcpy to
% copy and verify this Unique ID. We manipulate the stack within the interruption
% and modify the Unique ID while the memcpy is reading it from the monitored
% region.


% In this section, we make our attack more generalized by leveraging the DWT
% unit, Instead of only targeting on the invoke of a simple 
% function, we generalize our attack to hijack a large size dataset. 


==> attack/fpb_rom.tex <==
We further study the effects of our attack in a SEGGER J-Link v10 debug probe
unit. The J-Link v10 is based around an NXP LPC4322 microcontroller which
serves as the bridge between the device being debugged and a personal computer
running development software. These debug probes are among the most popular
used today. Some of these probes retail for over 1500 USD. As such, SEGGER adds
anti-counterfeit measures to the software running on the microcontroller to
avoid clones. In this section, we demonstrate how we can utilize the FPB in the
NXP LPC4322 to bypass these measures, bypassing the copy protection
mechanism\footnote{We presented a portion of this work at a recent hacker
forum and will include proper citation of this work upon acceptance.}.

% To show the validity of our attack, we choose the NXP chipset as the
% demonstrated platform. The NXP LPC435x/3x/2x/1x chipsets are designed for
% embedded applications based on ARM Cortex-M4 microcontrollers. Among the NXP
% LPC435x/3x/2x/1x series chipsets, LPC4322 is widely used in industry products,
% for example, SEGGER J-Link v10. The SEGGER J-Links are most widely used line of
% debug probes available today. In this section, we demonstrate the
% details of our FPB attack on NXP LPC4322 processor and bypass the copy
% protection of SEGGER J-Link. 

To produce a counterfeit device of this type hardware, a person has to reverse
engineer the target's hardware design. Then, the firmware from the device is
extracted. Firmware locked away by fuses can still be extracted, as the
technology to restore the fuses exists. When the hardware has been
reverse engineered and the firmware extracted, all that is left is to make a
clone device.

% The way piracy produce a illegal copy of licensed hardware product has some
% certain steps. They will reverse engineer the hardware design of target and try
% to extract the firmware of the hardware product. Even the setting of fuses can
% help to protect the firmware to be extracted, however the technology that
% restore the fuses has been well developed. With the exact same hardware and
% software, there is no reason the illegal copy of this hardware product cannot
% run.

SEGGER understandably wishes to prevent the J-Link from being cloned, as such,
they developed a mechanism that leverages the \emph{Unique ID} feature of the
NXP LPC4322 microcontroller \cite{lpc4322}. Each LPC4322 manufactured by NXP
includes a unique identification number, which is embedded into the device. No
two LPC4322 share the same number. Furthermore, the unique ID is stored in an
immutable place in the device and can not be overwritten. The LPC4322 also
provides In-Application Programming (IAP) routines in the Boot ROM. IAP
functions are provided to applications using an entry address at
\texttt{0x10400100}, alongside different parameters as commands. For example
passing parameter 51 as the first argument will copy the contents of RAM to
Flash, and parameter 58 to read the device's Unique ID.

% To prevent the products been cloned, the SEGGER J-Link develops a more advanced
% anti-clone mechanism by leveraging the Unique ID feature of NXP LPC4322
% processors.   To improve the security of products, the NXP LPC4322 includes a
% Unique ID for each manufactured processor. There is no two same Unique ID
% existing on different LPC4322 chips. Furthermore, the Unique ID is stored in
% the immutable place within the chip. NXP LPC4322 processor provide the
% In-Application Programming (IAP) routines in the Boot ROM. The IAP function is
% provided to user space application as a fixed function pointer address,
% \texttt{0x10400100} along with different parameters as different commands, for
% example, use number 51 as parameter to copy RAM to Flash, or 58 to read device
% Unique ID. In summery, to get the Unique ID within the embedded system,
% programmer should use \texttt{0x10400100} as function pointer and invoke this
% function along with parameter 58. 

The SEGGER leverages the Unique ID feature of the LPC4322 to build an
anti-clone mechanism. Before the J-Link firmware executes, enabling the
microcontroller to actas a debug probe, it checks the J-Link license included
in the firmware. The license is file is computed with the RSA-PSS algorithm
and includes the Unique ID from the microcontroller as a seed.  The
when license verification runs, the IAP function to obtain the Unique ID is
invoked. If the firmware is extracted and placed in a different
microcontroller, then the device identification will fail and the firmware will
not execute.

With the FPB, we can bypass the verification process. We explain the mechanism
which we utilize to bypass the firmware from poweron.

As the SEGGER J-Link powers on, the bootloader on the LPC4322 starts to execute
and verifies the integrity of the firmware to be loaded. The verification
generates a signature and checks it. If the verification passes, then the
J-Link firmware will be executed. If a direct modification is made to the
firmware, the verification process fails and the firmware will not run. The
J-Link firmware proceeds to verify the license in the firmware by performing a
call to read the LPC4322's Unique ID using command 58 in the IAP function. The
license is verified using RSA-PSS. However, with the FPB active, we can hijack
control-flow during this process. We hook into the IAP function inserting a
branch instruction to a function where we return a fake Unique ID.

The J-Link firmware uses a dereference to obtain the entry point of the IAP
function and then branch to it. The code takes the following simplified form:

\begin{lstlisting}[language=C, style=c]
ldr r2, [pc, #offset]
bx r2
...
.word 0x10400100
\end{lstlisting}

We set up a data literal comparator to point to the address where the loaded
literal resides. The corresponding entry in the remap table is made to point to
a \texttt{do\_fake\_dispatch()} function which returns a fake Unique ID if
parameter 58 is passed, and dispatches all other functions to the IAP itself.
This procedure is summarized as follows.

\begin{lstlisting}[language=C, style=c]
	#define IAP_LOCATION (0x10400100);

	int remap_table[8];

	void do_fake_dispatch(int *para, int *rp_value) {
		/* Read the Unique ID  command */
		if (para[0] == 58) { 
			*rp_value = fake_unique_id;
		} else {
			/* dispatch IAP function */
			(void(*)(int*,int*))IAP_LOCATION(para, rp_value)
		}
		return;
	}

	void enable_do_fake_dispatch(void) {
		remap_table[6] = 
			(unsigned int)do_fake_dispatch; 
		FPB->REMAP = (unsigned int)remap_table;
		FPB->CTRL = 0x00000003;
		FPB->COMP[6]=(LITERAL_VALUE_LOCATION|0x00000001);
		resume_chip_boot();
	}
\end{lstlisting}

We then assemble this code and inject it into a blank region of flash memory.
By using a programmer, we modify the reset handler of the vector table of the
LPC4322 bootloader into the address of our
\texttt{enable\_do\_fake\_dispatch()} function. This way, every time the
microcontroller boots, the FPB will be setup. Because we are able to redirect
control-flow in the J-Link firmware without modifying it, and because we are
able to return a cloned Unique ID, the firmware can freely be transferred
accross devices. 


==> attack/rtos_v2.tex <==
%%% TODO: change back to old section, reuse some of this material in old
%%% section

We now show how we can utilize the recent TCP/IP out of bounds write
vulnerability found in FreeRTOS \cite{CVE-2018-16528}. The vulnerability was
not only present in the FreeRTOS source tree, but also in Amazon's AWS
FreeRTOS, and WHIS OpenRTOS and SafeRTOS, the latter of which is certified for
use in safety critical systems. The error occurs in the way the TCP/IP handler
decodes incoming packets, by blindly trusting the size field in the packet
header. An attacker can send a malformed TCP/IP packet to a device running the
vulnerable stack and overwrite up to \SI{64}{\kibi\byte} outside the buffer
allocated by FreeRTOS.

This vulnerability is trivially exploitable by corrupting a code pointer held
in SRAM. However, we opt to weaken the attacker's power by choosing to act
under the following conditions: (1) a CFI defense is in place, so no code-reuse
attacks are possible; and (2) tasks in the RTOS are executed using a least
privileged model, such as the one presented in uVisor. Our objective is to
undermine all protection mechanism provided by the system and gain persistence,
that is, we wish disable the MPU and to gain arbitrary control-flow.

We note that the TCP/IP stack is integrated with the HAL in FreeRTOS. As such,
it runs at privileged level. Unfortunately, we are limited to the amount of
data we can send to the device by two factors, the network's maximum
transmission unit (MTU), and the maximum size of the TCP/IP packet. In real
life scenarios, the MTU will likely be the limitant, as it is usually smaller
than the maximum packet size. Regardless, we are unable to utilize the
vulnerability as is to corrupt the FPB registers, as these are found in the
Private Peripheral Bus area of the memory map.

%% TODO: not there yet
To overcome this limitation we are performing analysis on a compiled FreeRTOS
binary to find which variables are allocated in the area where corruption can
occur. The idea behind this is to turn the overflow into a controlled write
that allowed us to corrupt the FPB registers. The remap table itself can be
injected as data in the TCP/IP packet.
%% TODO: remove this portion
Unfortunately, at this time we have been
unable to achieve a controlled write that allows us to reliably corrupt the FPB
registers. We see data being corrupted leading to crashes, signaling that
critical OS data structures are being corrupted. We believe that with further
experimentation we can obtain the desired results. As such, we will keep
working on the attack and update the paper with more results as they become
available. Furthermore, we will give more details on the data flow technique
used in the technical report. 


% We further experiment with ARM mbed uVisor. Imperative to the uVisor model is
% that the privileged Hardware Abstraction Layer (HAL) is assumed to be trusted.
% 
% Since applications can not access anything outside their access control list,
% we must consider vulnerabilities in uVisor or the HAL. For this purpose, we
% developed a vulnerable driver for uVisor and added it to our local source tree.
% The driver performs an out of bounds write due to insufficient sanitation of
% inputs. The vulnerability is exposed to unprivileged software by means of the
% supervisor call interface, and a corrupted object being sent to the device. The
% registered handler must temporarily raise privileges to run HAL code and
% perform the load. For our demonstration, we create two containers on top of
% uVisor. One of them gathers user input and stores it in a buffer, the other one
% performs a request to load bitmaps through the supervisor call interface. Both
% containers do not perform any type of inter-process communication, and as per
% uVisor model both tasks are isolated from each other.
% 
% Our objective is to undermine the protection mechanism provided by uVisor,
% that is we wish to disable the MPU and have unfettered access to the entire
% device. For this end, we utilize the container that gathers user input to
% inject the remap table with the encoding for the instructions that disable the
% MPU. The injected instruction stream is similar to the one covered in Figure
% \ref{fig:arbitrary_exec_mpu_disable}. Using the container that receives
% bitmaps, we tamper with the FPB registers using the vulnerability in the HAL
% being exposed by the supervisor call interface. We point the \texttt{FP\_REMAP}
% register to the buffer used in the user input container and set the comparator
% registers to the addresses containing the routines that handle the MPU when
% switching containers. Because the FPB ignores MPU permissions, it is capable of
% providing instructions from the memory space of the user input container. With
% the MPU permanently disabled, we are once again free to arbitrarily inject code
% and execute it, as well as read any memory location.
% 
% During our testing, we noted that if we enabled the FPB too early, the system
% would go on to exhibit odd behavior, sometimes triggering a hard fault, and
% sometimes executing seemingly random code. This is because the remap table had
% not been fully loaded to memory, resulting in the comparator registers trapping
% instructions and then using an undefined instruction stream to patch. Because the
% processes did not have any built-in synchronization, our solution to this was
% to ensure that the remap table had been fully loaded before triggering the
% system call that enabled the FPB.

% We should note that at the time of writing, uVisor is being phased out in favor
% of the ARM Platform Security Architecture (PSA) \cite{arm_psa}. Currently,
% development efforts for ARM PSA are targeting the ARMv8-M architecture, which
% provides an embedded version of the ARM Security Extensions (popularly known as
% TrustZone-M). To the best of our knowledge, at this time there is only one
% commercially available microcontroller that implements this version of the ARM
% ISA, the Microchip SAM L10/11 family of microcontrollers which are developed
% around an ARM Cortex-M23 core. As noted in Section \ref{sec:discussion},
% microcontrollers that offer TrustZone-M do not offer the ability to remap flash
% addresses with the FPB.
% 


==> attack/segger.tex <==
\subsection{Overview of the J-Link v10 Debug Probe}
The SEGGER J-Link v10 debug probe is built around the NXP LPC4322
microcontroller. Each LPC4322 includes a unique identification number which is
embedded in the device at manufacturing time.
%No two LPC4322 share the same number.
Furthermore, this Unique ID is stored in an immutable place in the
device. Moreover, the LPC4322 also provides a read only memory containing boot
code and a series In-Application Programming (IAP) routines. The IAP entry
point is located at address \texttt{0x10400100}. The function at this address
takes a variable number of arguments. The first one is used to dispatch a
service from the IAP routines. For example, the value 51 corresponds to a
routine which copies the contents of RAM to Flash; and the value 58 as the
first parameter prompts the IAP to read the device's Unique ID. 

When the J-Link powers on, the Cortex-M4 core in the LPC4322 microcontroller
starts its power-on reset procedure. The CPU initializes itself using the
contents of the vector table and starts execution.
%The CPU enters handler mode and 
%sets its initial hardware state by storing the contents of address
%\texttt{0x00000000} into the main stack pointer register, \texttt{msp}, and the
%contents of address \texttt{0x00000004} into the program counter register,
%\texttt{pc}. The CPU exits handler mode and execution resumes from the address
%loaded into \texttt{pc}.
When examining the LPC4322 memory map we see that execution starts from the
on-chip ROM. Here, a bootloader verifies the integrity of the firmware by
utilizing a simple checksum algorithm. The computed checksum is compared to the
expected one, which is stored alongside the firmware in the on-chip flash.

Once this verification passes, the J-Link firmware starts to execute and
performs the validation procedure for the license. This uses the RSA-PSS
signature algorithm and uses the LPC4322's Unique ID as a salt. This ties the
firmware to the device in which it is being run, as a different device ID would
generate the incorrect signature. The firmware uses IAP function 58 to obtain
the Unique ID. Clone or counterfeit devices could attempt to bypass the
signature verification process by patching the binary, but this requires an
ongoing effort on binary analysis on the counterfeiter's part for every
firmware update released by SEGGER, who obfuscates their binaries to deter
reverse engineering efforts.

\subsection{Bypassing Firmware Verification}

With the FPB, we can bypass the verification process without the need to
reverse engineer the entire signature algorithm. By hijacking control-flow
during the call to obtain the Unique ID, we can present the signature
computation process with a Unique ID of our own choosing. The J-Link firmware
uses a dereference to obtain the entry point of the IAP function and then
branch to it. This takes the simplified form:
\begin{lstlisting}[style=arma]
ldr r2, [pc, #offset]
bx r2
...
.word 0x10400100
\end{lstlisting}

We set up a data literal comparator to point to the address where the loaded
literal resides. The corresponding entry in the remap table is made to point to
a \texttt{do\_fake\_dispatch()} function which returns a fake Unique ID if
parameter 58 is passed, and dispatches all other functions to the IAP itself.
We list the modified procedure in Appendix \ref{sec:lpc_dispatch_override}.
We assemble this code and combine it with the firmware of the J-Link, change
the dispatch address of the bootloader to our
\texttt{enable\_do\_fake\_dispatch()} function, compute a new bootloader
checksum, and place it on a different LPC4322 microcontroller.  When powered
on, the bootloader checks pass, our code executes storing our FPB
configuration, and then transitions to the J-Link code.  The J-Link proceeds to
perform the license verification procedure. However, when it attempts to obtain
the Unique ID through the IAP procedure, our dispatcher returns that of the
original LPC4322 resulting in the signature check to succeed.

% This way, every time the
% microcontroller boots, the FPB will be setup. Because we are able to redirect
% control-flow in the J-Link firmware without modifying it, and because we are
% able to return a cloned Unique ID, the firmware can freely be transferred
% accross devices. 


==> figs/fpb_base_address.tex <==
\usetikzlibrary{positioning}

\lstset{%
  frame            = tb,    % draw frame at top and bottom of code block
  tabsize          = 1,     % tab space width
  numbers          = left,  % display line numbers on the left
  numberstyle      =\tiny,
  numbersep        =5pt,
  framesep         = 6pt,   % expand outward
  framerule        = 0.4pt, % expand outward 
  backgroundcolor  = \color{yellow!30}, % backgroundcolor color
  showstringspaces = false,              % do not mark spaces in strings
}

\begin{lstlisting}[language = c, escapechar = !,
    basicstyle = \ttfamily\bfseries, linewidth = 0.75\linewidth,
    xleftmargin=0.05\columnwidth] 
    ldr r0,!
        \tikz[remember picture] \node [] (a) {};
    ![pc, #offset]

    ldr r0, [r0, r1]

    .word array_base!
        \tikz[remember picture] \node [] (b) {};
\end{lstlisting}

\begin{tikzpicture}[remember picture, overlay,
    every edge/.append style = { ->, thick, >=stealth,
                                 dotted, line width = 1pt },
    every node/.append style = { align = center, minimum height = 10pt,
                                 font = \bfseries, fill= green!20},
                  text width = 2.5cm ]
    \node [above left = .75cm and -.75 cm of a,text width = 2.2cm]
                             (A) {GOAL: change base address};
    \node [right = 1.cm of b, text width=2.5cm, text centered]  (B) 
    {Set FPB\_COMP0 to array\_base}; 
    \node [below left = 0.1cm of B, text width=2.5cm, text centered] (C) 
    {Set FPB\_REMAP6 to fake\_array\_base};
    \draw (A.south) + (0, 0) coordinate(x1) edge (x1|-a.north);
    \draw (B.west) edge (b.east);
    \draw (B.south) edge (C.east);

    %\node[rectangle, minimum height=5.5cm, minimum width=8cm] at (0,1) {};
\end{tikzpicture} 


==> figs/regions.tex <==
\draw (-1, 4.898437498603016) -- ++(2, 0);

\draw[gray] (-1, 0.375) -- (-2.5, -0.3);
\draw[gray] (-1, 0.3759765625) -- (-2.5, 0);
\node[
		text width=3cm,
		text centered,
		anchor=east,
		inner sep=0cm,
		draw, rectangle,
		minimum height=0.3cm,
		fill=gray!20,
	] at(-2.5, -0.15) {\footnotesize\SI{1}{\mebi\byte} bit band region};

\draw[gray] (-1, 0.421875) -- (-2.5, 0.125);
\draw[gray] (-1, 0.46874999860301614) -- (-2.5, 1.125);
\node[
		text width=3cm,
		text centered,
		anchor=east,
		inner sep=0cm,
		draw, rectangle,
		minimum height=1cm,
		fill=gray!20,
	] at(-2.5, 0.625) {\footnotesize\SI{32}{\mebi\byte} bit band alias};

\draw[gray] (-1, 0.375+0.75) -- (-2.5, 1.25);
\draw[gray] (-1, 0.3759765625 + 0.75) -- (-2.5, 1.55);
\node[
		text width=3cm,
		text centered,
		anchor=east,
		inner sep=0cm,
		draw, rectangle,
		minimum height=0.3cm,
		fill=gray!20,
	] at(-2.5, 1.4) {\footnotesize\SI{1}{\mebi\byte} bit band region};

\draw[gray] (-1, 0.421875+0.75) -- (-2.5, 1.675);
\draw[gray] (-1, 0.46874999860301614+0.75) -- (-2.5, 2.675);
\node[
		text width=3cm,
		text centered,
		anchor=east,
		inner sep=0cm,
		draw, rectangle,
		minimum height=1cm,
		fill=gray!20,
	] at(-2.5, 2.175) {\footnotesize\SI{32}{\mebi\byte} bit band alias};

\draw[gray] (-1, 4.875) -- (-2.5, 4.725);
\draw[gray] (-1, 4.898437498603016) -- (-2.5, 5.025);
\node[
		text width=3cm,
		text centered,
		anchor=east,
		inner sep=0cm,
		draw, rectangle,
		minimum height=0.3cm,
	] at(-2.5, 4.875) {\footnotesize Private Peripheral Bus};

